Upper Bounds for Totally Symmetric Sets

Totally symmetric sets are a recently introduced tool for studying homomorphisms between groups. In this paper, we give full classifications of totally symmetric sets in certain families of groups and bound their sizes in others. As a consequence, we derive restrictions on possible homomorphisms between these groups. One sample application of our results is that any homomorphism of a braid group to a direct product of solvable groups must have cyclic image.

==> TODO.tex <==
\section{TODOs}
\begin{itemize}
    \item Section summaries in the introduction
    \item write sections 5 and 6
\end{itemize}

\section{New Section Outline}
\begin{itemize}
    \item Introduction
    \item Totally Symmetric Sets
    \item Specific Groups: Abelian, Free, Dihedral, Baumslag-Solitar (Caleb)
    \item Products: Semi-direct of cyclic groups, direct product, free product (Caleb)
    \item Bounds Derived Through SES: SES, Solvable groups, odd order groups (Lily)
    \item homomorphisms
\end{itemize}




